Welfare Analysis of Network Neutrality Regulation

Consumers of Internet content typically pay an Internet Service Provider (ISP) to connect to the Internet. A content provider (CP) may charge consumers for its content or may earn via advertising revenue. In such settings, a matter of continuing debate, under the umbrella of net neutrality regulations, is whether an ISP serving a consumer may in addition charge the CPs not directly connected to the ISP for delivering their content to consumers connected to the ISP. We attempt an answer by looking at the problem through the lens of a regulator whose mandate is to maximize the cumulative welfare of ISPs, CPs, and consumers. Specifically, we consider a two-sided market model, in which a local monopoly ISP prices Internet access to consumers and possibly to CPs as well. The CPs then decide whether to enter a competitive but differentiated market and the consumers decide whether to connect to the ISP. Unlike prior works, we model competition between the CPs together with consumer valuation of content and quality-of-service provided by the ISP. We do so by using a novel fusion of classical spatial differentiation models, namely the Hotelling and the Salop models, in addition to simple queue theoretic delay modeling. Via extensive simulations, we show that the equilibrium in the non-neutral setting that allows an ISP to charge a CP welfare-dominates the neutral equilibrium.

==> model_bak.tex <==
\section{Basic Model}
%\section{Modeling }
\label{sec:model}
%SKK: We are sort of saying what is in the footnote in the intro. Specifically that CPs don't pay... in the larger network \footnote{Typically, as \cite{economides2012network} have noted, consumers are more locationally constrained than the CPs. As a result, while CPs have negotiated a very low price for network access from their originating ISP and do not pay at all to the rest of the ISPs for last mile access, the consumers end up paying a lot more.}
There is a monopoly ISP and many potential CPs for whom this ISP is not the originating ISP. Introduce the interval $[0,1]$ as the \emph{Hotelling} line of the standard horizontal product differentiation model for the ISPs. Let the ISP be located at the left extremity, location $0$, of this line. There is a continuum of consumers uniformly distributed on the Hotelling line. Let the product differentiation parameter for the ISP be normalized to $1$. Non-price factors therefore impose a cost of $x$ on a customer at location $x$ on the Hotelling line.

Let $t \in (0,1)$ be the product differentiation parameter for the CPs. Note that we restrict $t<1$. This is to capture the fact that it is easier to substitute between CPs than it is to substitute between ISPs. Let $y$ be the distance travelled by a consumer to connect to a CP. This imposes a cost of $ty$ on the consumer. Consumers cannot connect to the CPs without first connecting to the ISP. The CPs space themselves equidistantly on a Salop circle whose perimeter, as we detail soon, is determined by the customers that choose to connect to the ISP. 

All CPs provide free content to the consumers; their only source of revenues is from advertising. Let $r$ be the advertising revenue per consumer, same for all CPs. Let $d$ be the access price charged by the ISP to the consumer. Let $f$ be the fixed cost of entering the provider market for any CP.
%\footnote{This relative specification of the product differentiation parameters is motivated by their interpretation as the ease of substitution between the products. It is much easier to substitute between CPs than it is to substitute between ISPs.}We must model the total time required to fulfill a consumer's request, which is the sum of the time a request waits for service by the ISP and the time it spends getting serviced.

Consumers pay a congestion cost, which is the average time the ISP takes to fulfill a consumer's request for content. To capture this, we model the ISP as a M/M/1~\cite{gross1998fundamentals} service facility. Specifically, following~\cite{pil2010net}, we assume that the aggregate demand for content from consumers created at the ISP is well modeled by a Poisson process of rate $\lambda$ per unit length of the single dimension containing consumers connected to the ISP. Further, the time taken by the ISP to service a consumer's request for content is exponentially distributed with a mean service time of $1/\mu$. We assume $\lambda < \mu$, which is required for the average time to fulfill a request to stay bounded. Finally, consumer requests are serviced by the ISP in a first-come-first-served manner. This means that a request that arrives at the ISP must wait for requests that arrived earlier to finish obtaining service from the ISP. 

Consumer monetary valuation of the total requested content is $v$. In the non-neutral regime, the ISP can charge the CPs for servicing requests for their content at an access price of $a$. In contrast, the neutrality regime prohibits the ISP from charging the CPs a price when it is not the originating ISP for them, which we assume is the case here. The two regimes therefore induce different market games through which the entities interact.

%Following \cite{pil2010net}, we model congestion in the ISP's network using the standard M/M/1 queueing model of operations research. The rate at which each consumer requests content follows a Poisson process with hazard rate $\lambda > 0$. Let $\mu$ denote the network capacity of the ISP. The time to service content request is exponentially distributed with a mean of $1/\mu$.  We assume that $\mu > \lambda$ so that the steady state expected waiting time is well defined. Consumer monetary valuation of the total content he requests is $v$.

\subsection{Non-neutral Regime}

\begin{figure}
	\centering
	\includegraphics[width=0.9\columnwidth]{Figures/Fig_1.pdf}
	\caption{\small{Left Panel shows the \emph{Hotelling} line for the ISP dimension. Right panel shows the folded \emph{Hotelling} line segment of length $\hat{x}$ as the \emph{Salop} circle with the same circumference. It also shows the symmetric alignment of CPs when $n=4$ for when the customer at $\hat{x}$ travels a distance $\hat{x}/(2n) = \hat{x}/8$ to reach a CP.}}
	\label{fig:ModFig}
\end{figure}

In the non-neutral regime, the ISP, the CPs and the consumers interact through the following \emph{multi-stage game}:  
\begin{enumerate}%[leftmargin=0pt]
\item ISP chooses the access prices: $a$ for CPs and $d$ for consumers.
\item Consumers then choose whether to connect to the ISP.
\item CPs who are considering entering the market then simultaneously decide whether to enter or not. Suppose $n$ is the number of CPs who chose to enter. The CPs locate equidistantly\footnote{We follow \cite{salop1979monopolistic} in making the assumption of symmetric alignment of CPs on the Salop circle to focus on the entry decisions of CPs.} on a \emph{Salop} circle whose perimeter is the length $\hat{x}$ of the initial segment of the \emph{Hotelling} line on which consumers connect to the ISP.
\item Consumers who have connected to the ISP then connect to a CP and consume content. 
\end{enumerate}

We specify utility of a consumer who travels a distance $x$ on the \emph{Hotelling} line to connect to the ISP and distance $y$ on the \emph{Salop} circle to connect to the CP as
\begin{equation}\label{eqn:consumerUtil}
u = v - x  - ty - d - \frac{1}{\mu- \lambda \hat{x}},               
\end{equation}
where $\lambda \hat{x}$ is the aggregate rate of request for content from the length $\hat x$ of consumers. The last term in the expression for consumer utility $u$ is the congestion cost faced by a consumer. It is the resulting expected time the ISP takes to fulfill a consumer's request (called waiting time in~\cite{gross1998fundamentals}), given the demand $\lambda \hat{x}$.

%Specifically, it is the expected delay between request and delivery of content. It is the steady state expected waiting time \footnote{ See \cite{gross1998fundamentals} for detailed derivations and more on queueing theory}. 

We specify ISP's profit as $\pi(d, a) = d \hat{x} + na$. We specify profits of $\text{CP}_i$ as $\pi_i = r D_i - a - f$, where $D_i$ is the demand that $\text{CP}_i$ faces. 

To determine this demand $D_i$ we must decide how the CPs are aligned on the Salop circle relative to the marginal consumer at $\hat{x}$ who connects to the ISP. This is important for it determines the distance traveled by this consumer on the Salop circle and therefore affects the location $\hat{x}$ on the Hotelling line. Two extreme cases are possible. In one, illustrated in Figure~\ref{fig:ModFig}, the marginal consumer travels a distance $\frac{\hat{x}}{2n}$; in the other, the consumer travels no distance, that is a CP locates itself at $\hat{x}$. %
%These cases are depicted in the Figure~\ref{fig:ModFig}.There is a modeling issue to be resolved- how are the CPs aligned on the Salop circle relative to the marginal consumer at $\hat{x}$ who connects to the ISP. This is important for it determines the distance traveled by this consumer on the Salop circle and therefore affects the location of $\hat{x}$ on the Hotelling line. Two extreme cases are possible. In one, the marginal consumer travels a distance $\frac{\hat{x}}{2n}$; in the other, he travels no distance at all. These cases are depicted in the Figure~\ref{fig:ModFig}.
One could introduce an extra parameter $\beta \in [0,1]$, and specify the distance traveled by the marginal consumer as $\frac{\beta \hat{x}}{2n}$. The extreme cases correspond to the values $\beta = 1$ and $\beta = 0$. We will, however, choose $\beta = 1$ in our analysis for two reasons. First, any $\beta \in (0, 1]$ retains the structural feature that demand on either side (whether $\hat{x}$ or $n$) responds to prices ($d$ and $a$) on both sides. Therefore $\beta = 1$ carries the flavor of analysis of any $\beta \in (0,1)$. Second, as will be clearer from analysis that follows, $\beta = 0$, kills any dependence of $\hat{x}$ on $a$ and in that sense is a special case.

%One way to resolve this, at the cost of introducing and carrying around an extra parameter $\beta \in [0,1]$, is to specify the distance traveled by the marginal consumer as $\frac{\beta \hat{x}}{2n}$. The extreme cases correspond to the values $\beta = 1$ and $\beta = 0$. We will, however, focus on Extreme Case I i.e. $\beta = 1$ in our analysis for two reasons. First, any $\beta \in (0, 1]$ retains the structural feature that demand on either side (whether $\hat{x}$ or $n$) responds to prices ($d$ and $a$) on both sides. Therefore $\beta = 1$ carries the flavor of analysis of any $\beta \in (0,1)$. Second, $\beta = 0$ i.e. Extreme Case II kills any dependence of $\hat{x}$ on $a$ \footnote{This will become clear in a while from analysis.} and in that sense is a special case. 
 
To summarize, the parameters of the model are the consumer valuation $v$, the advertising revenue $r$, the normalized product differentiation parameter $t$, fixed CP costs $f$, the rate of content request $\lambda$, and the service rate $\mu$. The choice variables are the prices $a$, $d$, the entry decisions of the CPs, and the consumer decisions with regards to connecting to the ISP and the CPs. The solution concept used to analyze the model is subgame perfect Nash equilibrium. We will use the backward induction algorithm to find subgame perfect Nash equilibria of the multi-stage game.

%$ v, r, t, f, \lambda, \mu$ and the choice variables are $a$, $d$, the entry decisions of the CPs and the consumer connection decisions to the ISP and CPs. The solution concept used to analyze the model is subgame perfect Nash equilibrium. We will use the backward induction algorithm to find subgame perfect Nash equilibria of the multi-stage game.

Suppose we are in the subgame in which the mass of consumers who chose to connect to the ISP is $\hat{x}$, the number of CPs who chose to enter is $n$ and they place themselves symmetrically on the \emph{Salop} circle whose perimeter is $\hat{x}$. So $CP_i$ faces a demand $D_i = \frac{\hat{x}}{n}$ with consequent profits
\begin{equation}
\pi_i = r \frac{\hat{x}}{n} - f - a.
\end{equation}
Under free entry, the optimal number of CPs who enter is determined by the zero-profit condition yielding
\begin{equation}\label{CPDemand}
n = \frac{r \hat{x}}{a+f}.
\end{equation}
Ceteris paribus, an increase in ISP's access price $a$ to CPs just adds to their fixed costs and reduces the number of CPs which enter the market. Similarly, an increase in total demand $\hat{x}$ encourages entry.

The marginal consumer at $\hat{x}$ travels a distance $\frac{\hat{x}}{2n}$ and is indifferent between connecting to the ISP and not connecting to it, that is it has a utility of $0$. Setting the utility $u$ in~(\ref{eqn:consumerUtil}) to zero, we can write 
\begin{equation*}
v - \hat{x} - \frac{t \hat{x}}{2n} - d - \frac{1}{\mu- \lambda \hat{x}} = 0.
\end{equation*}

Using $n$ from Equation~(\ref{CPDemand}) in the above equation, we have 
\begin{equation}   \label{ConDemand}
v - \hat{x} - \frac{t (a+f)}{2r} - d - \frac{1}{\mu- \lambda \hat{x}} = 0.
\end{equation}
Let $\hat{x}(d, a)$ solve Equation (\ref{ConDemand}). Then 
\begin{align}
\hat{x}(d, a)  &= \frac{1}{2\lambda}\left(\mu + \lambda \big(v-d - \frac{t (a+f)}{2r} \big)\right.\nonumber\\
&\left.- \sqrt{[\mu - \lambda \big(v-d - \frac{t (a+f)}{2r} \big)]^2 + 4 \lambda}\right). \label{Demand1}
\end{align}
Further, using~(\ref{CPDemand}), we can calculate the number of CPs
\begin{align}
n(d, a) &= \frac{r \hat{x}(d, a)}{a+f}.  \label{Demand2}
\end{align}
So the total demand on either side is decreasing in both the access prices. 

The ISP chooses the access prices $d$ and $a$ to maximize its profits subject to the constraints that the resulting consumer demand is nonnegative and the demand on the CP side is at least 1. Formally it faces
\begin{align*}
[OPT1] \quad \quad  \max_{d, a} \quad \pi(d, a) &= d \hat{x}(d, a) + a n(d,a) \\
\text{subject to } \quad 0 \le \hat{x}(d, a) &\le 1,   \\
n(d,a) &\ge 1.
\end{align*}

Define $e(\hat{x}(d, a), d) := - \frac{\ud \hat{x}(d, a)/ \hat{x}(d, a)}{\ud d/ d}$ to be the elasticity of consumer demand $\hat{x}(d, a)$ with respect to $d$. Similarly, define $e(\hat{x}(d, a), a)$ as the elasticity with respect to $a$. Let $e(n(d, a), d)$ and $e(n(d, a), a)$ be the corresponding elasticities of the number of CPs. Then an unconstrained optimum is a solution to the following pair of equations in $(d, a)$.

%Let $e(\hat{x}(d, a), d)$ \footnote{$e(\hat{x}(d, a), d):= - \frac{\ud \hat{x}(d, a)/ \hat{x}(d, a)}{\ud d/ d}$} and $e(\hat{x}(d, a), a)$ be the elasticities of consumer demand $\hat{x}(d, a)$ with respect to $d$ and $a$ respectively. Let $e(n(d, a), d)$ and $e(n(d, a), a)$ be the corresponding elasticities of CP demand. Then an unconstrained optimum is a solution to the following pair of equations in $(d, a)$. 
\begin{align}
e(\hat{x}(d, a), d) + \frac{an}{d \hat{x}} e(n(d, a), d) &= 1,   \label{FOC_d} \\
e(n(d, a), a) + \frac{d \hat{x}}{an} e(\hat{x}(d, a), a) &= 1.   \label{FOC_a}
\end{align}

Equations (\ref{FOC_d}) and (\ref{FOC_a}) can be interpreted as follows. If the monopolist ISP wants to increase $d$, he faces the traditional margin vs volume tradeoff. That is, he loses some consumers but makes more on the existing consumers. However, since the ISP is operating in a two-sided market, an additional effect arises via network externalities. A decreases in consumer market size makes entry unattractive for CPs. So the provider market size decreases which reduces the ISP's revenues from that market. Similarly, if the ISP wants to increase $a$, in addition to facing the traditional margin vs volume tradeoff \SKK{The trade-off is unclear and uses terminology that is unfamiliar to me. Also, while the interpretation of the equations is clear, it is not apparent how the interpretation follows from the equations.} in the provider market, it has to consider that increasing $a$ also decreases the consumer market size which has a second order effect on further reducing volumes in the provider market. The optimal access prices $(d, a)$ balance these effects simultaneously. 

\subsection{Net Neutrality Regime}
Net neutrality regulation constrains the access price $a$ that the ISP can charge CPs to be zero. In the neutrality regime, the ISP, the CPs and the consumers interact through the same multi-stage game as in free market regime but with the constraint $a = 0$.    

The ISP faces the following optimization problem for choosing the access price to consumers
\begin{align*}
[OPT2] \quad \quad \max_{d} \quad \pi(d, a=0) &= d \hat{x}(d, a=0)   \\
\text{subject to } \quad 0 \le \hat{x}(d, a=0) &\le 1,   && (C_1)\\
n(d, a=0) &\ge 1,     && (C_2)
\end{align*}
where $\hat{x}(d, a=0)$ and $n(d, a=0)$ are found by setting $a = 0$ in Equations (\ref{Demand1}) and (\ref{Demand2}).

The unconstrained optimum of $[OPT2]$ is given by the value of $d$ at which the standard margin vs volume tradeoff \SKK{Unclear terminology; related to previous comment} in the consumer market is resolved optimally at
\begin{equation}   \label{NeutralOpt}
e(\hat{x}(d, 0), d) = 1
\end{equation}
and is the solution if it lies in the constraint set. The corresponding demands $\hat{x}(d, a=0)$ and $n(d, a=0)$ on both sides can be computed by setting $a=0$ and $d$ at its optimal value in Equations (\ref{Demand1}) and (\ref{Demand2}).

\subsection{Welfare}
\label{sec:Welfare}
The model we are studying is a transferable utility model. This implies that the cardinal welfare $W$ at any outcome is defined to be the sum total of consumers' surplus ($CS$), profits ($\pi_i$) of all CPs who enter and profit $\pi$ of the ISP. We have these expressions
\begin{align}
\pi &= d \hat{x} + na,    \nonumber  \\
\sum_{i=1}^n \pi_i &= r \hat{x} - nf - na,  \nonumber \\
CS &= \int_{0}^{\hat{x}} \big(v-d - \frac{1}{\mu- \lambda \hat{x}} -x \big) \ud x - \nonumber\\
&\quad n \int_{0}^{\hat{x}/n} ty \ud y  = \big(v-d-\frac{1}{\mu- \lambda \hat{x}} \big) \hat{x} - \frac{\hat{x}^2}{2} - \frac{t \hat{x}^2}{n}, \nonumber \\
W(\hat{x}, n) &= \pi + \sum_{i=1}^n \pi_i + CS = (v+r) \hat{x} -  \frac{\hat{x}^2}{2} - \frac{t \hat{x}^2}{n}\nonumber\\ &\quad - nf - \frac{\hat{x}}{\mu- \lambda \hat{x}}.  \label{Welfare}
\end{align}
The access prices cancel out because these are mere transfers from one party to another. The overall welfare in an equilibrium depends on the consumer market size and the number of CPs that populate the provider market. If the consumer market size $\hat{x}$ increases, consumer surplus and advertising surplus increase on account of more consumers being served but welfare decreases on account of two factors -- first, an increase in consumer market size increases the heterogeneity in consumer preferences which causes the product diversity along the ISP and the CP dimension to decrease relatively; second, an increase in consumer market size also increases the congestion cost for everyone. Similarly, an increase in the number of CPs who enter increases consumer surplus because there is more product diversity on the CP dimension for consumers but imposes greater fixed costs on the society.

As is standard in economic analysis, we compute the welfare optimum as a solution to the following problem.
\begin{align*}
[OPT3] \quad \quad \max_{\hat{x}, n} \quad & W(\hat{x}, n)   \\
\text{subject to } \quad 0 \le \hat{x} &\le 1,   \\
n &\ge 1.     
\end{align*}
The solution to $[OPT3]$ gives the size of consumer and provider market that is best from society's point of view when we have taken everyone's interest into account. 
